Pregelix: Big(ger) Graph Analytics on A Dataflow Engine

There is a growing need for distributed graph processing systems that are capable of gracefully scaling to very large graph datasets. Unfortunately, this challenge has not been easily met due to the intense memory pressure imposed by process-centric, message passing designs that many graph processing systems follow. Pregelix is a new open source distributed graph processing system that is based on an iterative dataflow design that is better tuned to handle both in-memory and out-of-core workloads. As such, Pregelix offers improved performance characteristics and scaling properties over current open source systems (e.g., we have seen up to 15x speedup compared to Apache Giraph and up to 35x speedup compared to distributed GraphLab), and makes more effective use of available machine resources to support Big(ger) Graph Analytics.

==> Makefile <==
TEX      := latex
PDFTEX   := pdflatex
BIBTEX   := bibtex
RM       := rm -f
OPTIONS  = -o
PDFTEXOPTIONS = --interaction batchmode

DVI     = pregelix.dvi
TARGET  = pregelix.pdf
BIBSRC  = $(shell ls *.bib)
BIBFILE = $(shell ls *.bbl)
EPSES =   $(shell ls figs/*.eps)
AUTOGEN_PDFS = $(addsuffix .pdf, $(basename $(EPSES)))


all: $(TARGET)

pregelix.pdf:  $(DVI)
	clear
	echo Running $(PDFTEX)
	$(PDFTEX) $(PDFTEXOPTIONS) $(basename $(DVI));\
	#open -a Preview pregelix.pdf

pregelix.dvi: $(AUTOGEN_PDFS) $(shell ls *.tex) reference.bib
	clear
	echo Running $(PDFTEX)
	echo $(basename $@)
	$(PDFTEX) $(basename $@)
	clear
	echo Running $(BIBTEX);\
	$(BIBTEX) $(basename $@) ;\
	clear;\
	for i in 1 2; do\
		echo Running $(PDFTEX);\
		$(PDFTEX) $(basename $@) ;\
        done

figs/%.pdf : figs/%.eps
	cd figs/  && GS_OPTIONS=-dAutoRotatePages=/None epstopdf $*.eps

pdfs: $(AUTOGEN_PDFS)

clean:
	$(RM) pregelix.pdf $(TARGET_PS)  $(DVI)  pregelix.aux pregelix.log *blg *~  $(basename $(TARGET)).out $(AUTOGEN_PDFS) .cache.*

view:	open -a Preview pregelix.pdf

clean:
	rm -f   *.aux *.bbl *.blg *.dvi *.log *.ps *.pdf

tidy:
	rm -f   *.aux *.bbl *.blg *.dvi *.log



==> src/approach.tex <==
In this work, instead of building a Pregel-like system from scratch, we explore an architectural alternative---expressing Pregel's semantics as database-style dataflows and executing them on a general-purpose data-parallel engine using classical parallel query evaluation techniques.  
We have used this approach to build Pregelix---a dataflow-based Pregel implementation for Big Graph analytics. Pregelix examines the value of a ``one-size-fits-a-bunch'' philosophy, demonstrating that a general execution engine can also support Big Graph analytics well.

The design and implementation of Pregelix explore and answer two research questions:  1. In order to efficiently support Big Graph analytics,  what the necessary extensibility does a data-parallel query execution engine need to provide?  2. Given an extensible data-parallel execution engine, how should one implement Pregel on top of it and what are the possible optimizations?


For the first research question,  there are two extensibility requirements for the query execution engine:

\begin{list}{\labelitemi}{\leftmargin=1em}\itemsep 0pt \parskip 0pt
\item Support for user-defined operators, such as reading/writing from distributed file systems and setting up user-defined (Pregel-specific) job contexts,

\item User-configurable task scheduling, with which one can implement sticky scheduling to leverage locally cached data on each cluster machine.

\end{list}

Based on these two requirements, 
we chose Hyracks~\cite{Hyracks} as the runtime execution engine for Pregelix.
%
Regarding the second research question, we have been exploring several key design issues:

\begin{list}{\labelitemi}{\leftmargin=1em}\itemsep 0pt \parskip 0pt
\item Pregel as dataflows.  Inside Pregelix, both vertices and messages are treated as tuples and Pregel's semantics are implemented by a query plan consisting of operators such as joins and grouped aggregations.

\item Vertex storage. We store vertices in partitioned B-trees, either using standard B-trees or LSM-trees (log-structured merge-trees).

\item Runtime choices.  Pregelix offers several logically equivalent runtime execution alternatives and allows users to choose among them.  Each alternative is implemented as data-parallel jobs.
\end{list}

==> src/contribution.tex <==
This work contains several key contributions. First, it demonstrates the feasibility of using a database-style approach to implement the Pregel model in a simple architecture.  Second,  we identified the extensibility requirements for a parallel query execution engine to support Big Graph analytics. Last but not least, we have released the Pregelix system (http://hyracks.org/projects/pregelix/) 
in open source form for use by the community.

==> src/dataflows.tex <==
\subsection{Vertex Storages}

\subsection{Join Strategies}

\subsection{Group-by Strategies}

\subsection{Redistribution Policies}

==> src/problem.tex <==
Recently, Google has proposed the Pregel programming
model~\cite{Pregel} for Big Graph analytics, where application programmers need no knowledge of parallel
or distributed systems. Instead, they just need to ``think like a vertex'' and write a few functions that encapsulate the logic for what one graph vertex does.
%
The vertex-oriented programming model has been found to ease the implementation of distributed graph algorithms to a great extent. 

There are several efforts (e.g., ~\cite{Giraph, GraphLab}) to build Pregel-like systems from scratch.
However, building such a system is complicated because a complete implementation must consider network issues, memory management, message delivery, parallel task scheduling,  fault-tolerance, vertex storage, and out-of-core support.  Moreover, if the system developer wants to support different runtime execution choices, doing that in the built-from-scratch world would add still more complexity.

